Complex Langevin: Correctness criteria, boundary terms and spectrum

The Complex Langevin (CL) method to simulate `complex probabilities', ideally produces expectation values for the observables that converge to a limit equal to the expectation values obtained with the original complex `probability' measure. The situation may be spoiled in two ways: failure to converge and convergence to the wrong limit. It was found long ago that `wrong convergence' is caused by boundary terms; non-convergence may arise from bad spectral properties of the various evolution operators related to the CL process. Here we propose a class of criteria which allow to rule out boundary terms and at the same time bad spectrum. Ruling out boundary terms in the equilibrium distribution arising from a CL simulation implies that the so-called convergence conditions are fulfilled. This in turn has been shown to guarantee that the expectation values of holomorphic observables are given by complex linear combinations of $\exp(-S)$ over various integration cycles. If the spectrum is pathological, however, the CL simulation in general does not reproduce the integral over the desired real cycle.

==> 5discussion.tex <==
\section{Discussion}
\label{limitations}

A remaining question is if our Assumption $A$ guarantees correctness of CL. What we 
showed is that it implies that there are no boundary terms and that the spectrum of $L_c$ lies in the left half of $\C$. 

But as stated in in \cite{trust} correctness also requires that $0$ is a {\em simple} i.~e. nondegenerate) eigenvalue of $L_c$ and $L_c^T$. It is obvious that 
$L_c$ and $L_c^T$ have at least one eigenvector with eigenvalue $0$: for $L_c^T$ it is 
$\psi_0 \propto \exp(-S)$ for $L_c^T$ and for $L_c$ a constant; in both cases the 
operators have to be defined on the original integration cycle to give the correct results.

Degeneracy can arise from the existence of inequivalent integration cycles. These 
connect different zeroes of $\rho(z)=\exp(-S(z)$, which may be finite or infinite, or 
they wind around compact directions of the configuration space. Inequivalent integration
cycles correspond to different eigenvectors, even though formally they are related by
analytic continuation. The `right' integration cycle is determined by the definition of the model, 
typically it is the real submanifold of the complexified configuration space, or a cycle 
equivalent to it.  

Nonergodicity of the CL process leads to degeneracy of the zero eigenvalue of $L^T$, 
the real Fokker-Planck operator, which will imply degeneracy for $L_c^T$ and $L_c$. The 
converse does not hold: there are examples where the CL process is ergodic, but 
the eigenvalue $0$ of $L_c^T$ is degenerate \cite{aarts_zeroes,salcse}.

Examples of non-ergodicity were found for simple models with zeroes in the complex 
density $\rho$ in \cite{aarts_zeroes}. But ergodicity may also fail in simple quartic 
models without finite zeroes, for instance for
\be
S=\frac{\lambda}{4}(z^2-(a+ib)^2)^2\,,\quad \lambda=2.\,,a=3.\,,b=1.\,,
\ee
where numerics strongly suggests that there are two different equilibrium distributions. In
this case there are two inequivalent integration cycles corresponding to different
directions in which $\rho=\exp(-S)$ goes to infinity; they may be chosen to agree with the
two stable Lefschetz thimbles. The CL simulation represents one of those, depending on the
starting point, whereas the real integration cycle corresponds to a linear combination of
the two. In this case there is a fix: by choosing starting points for CL with a suitable
probability distribution one may reproduce the real integration cycle.

This example shows the limitations of the criterion provided by our Assumption $A$, but
also of the ``drift criterion'' \cite{nagata}. Both criteria do not see the problems of
degeneracy of the eigenvalue $0$, whether for $L^T$ or for $L_c$. It should be noted that nonergodicity may also be difficult to spot even
in the case of the real Langevin method or in ordinary Monte Carlo simulations.  

The situation is similar if $\rho$ has finite zeroes on the original real integration
cycle. In the noncompact case, there are typically at least two inequivalent integration cycles, starting at that
zero and going to infinity in different directions; in the case of compact models, this happens if two zeroes can be connected in inequivalent ways.
In fact, one can then see easily that the eigenvalue $0$ of $L_c^T$ is
degenerate: we may multiply $\psi_0=\exp(-S)$ by the characteristic function of an interval
between two zeroes (one of which may be at infinity), thereby producing a new eigenfunction of $L_c^T$ with eigenvalue $0$. 

In \cite{aarts_zeroes} we found examples of this phenomenon, such as the one-link $U(1)$
model with $\kappa=2$ and $n_p=4$, defined by
\be
\rho(z)= (1+\kappa \cos(z))^{n_p}\exp(\beta \cos(z))\,.
\ee
Whether CL is ``correct'' here depends on the initial choice of the integration cycle
defining the model. $\rho$ has two zeroes, and we may choose as integration cycle either
one of the two inequivalent paths connecting the two different zeroes, or the closed path
winding around the the cylinder. The latter cycle can be written as the sum (or difference,
depending on the orientation) of the former two.

In these simple examples it turned out that the two ergodic components of the CL process
correspond to the two inequivalent cycles connecting the two zeroes of $\rho$. In this
sense one may say that CL is still correct, but does not reproduce the original cycle,
which is a superposition of the two inequivalent cycles.

In the case where the measure has zeroes on the complex plane,
it also happens in some cases that the CL process is ergodic, but does not represent any of the
integrals over the inequivalent cycles. Such an example is the one-pole model as discussed
in \cite{salcse} as well as \cite{aarts_zeroes}. It has two inequivalent cycles, connecting
the zero at the origin to either $+\infty$ of $-\infty$. In this case CL is ``not correct'' and there are boundary terms, as found in \cite{seiler}.

It is a general fact that in the absence of boundary terms the CL process will relax to an equilibrium measure satisfying the so-called consistency conditions \cite{etiol} 
\be
\bra L_c\cO\ket =0\,;
\ee
in \cite{salcse} it was shown that this implies that $\bra L_c\cO\ket$ is equal to a linear 
combination of the integrals over a basis of the complex integration cycles. 

In realistic models, such as QCD, what is a correct  integration cycle is dictated by physics; it is any cycle homologous to the real submanifold. 

Finally, the existence and uniqueness of the $L_c$ evolution of the observable is in
general an unsolved mathematical problem; the semigroup $\exp(tL_c)$ is not in all cases
well under control, so we cannot say in which sense it is ``correct''. But it might be
enlightening to look at the one-pole example studied in \cite{aarts_zeroes} and again in
\cite{seiler}, where we have an explicit expression for the integral kernel of that
semigroup.  In fact, as remarked there, there are even two different semigroups solving the same equation, but on different spaces. We discuss this in some detail in Appendix \ref{nonunique}.

If we attempt to generalize from this example, we conjecture that at a finite zero
there are always several solutions of the $L_c$ evolution. Which one is correct,
if any, depends on the original integration cycle defining the problem to be
solved by CL.

In a non-ergodic situation, in particular in the presence of poles, it may depend on 
the starting point of CL which integration cycle is represented. For lattice models it 
is no easy to determine all the possible integration cycles as well as the linear 
combination of them representing the original problem.

These thorny problems are not yet completely understood. A possible way forward may be the introduction of kernels into the CL method. Some first promising steps in this direction has been recently made in \cite{alvestad,Boguslavski:2022dee}. In this paper we have shown that barring ergodicity problems and problems of inequivalent integration cycles (which might appear in 
systems with zeroes of the measure on the complex plane), vanishing boundary terms or well behaved the control variables (defined above) imply the correctness of the 
expectation values of the Complex Langevin process.



